Automatic Generation of Precise and Useful Commutativity Conditions (Extended Version)

Reasoning about commutativity between data-structure operations is an important problem with applications including parallelizing compilers, optimistic parallelization and, more recently, Ethereum smart contracts. There have been research results on automatic generation of commutativity conditions, yet we are unaware of any fully automated technique to generate conditions that are both sound and effective. We have designed such a technique, driven by an algorithm that iteratively refines a conservative approximation of the commutativity (and non-commutativity) condition for a pair of methods into an increasingly precise version. The algorithm terminates if/when the entire state space has been considered, and can be aborted at any time to obtain a partial yet sound commutativity condition. We have generalized our work to left-/right-movers and proved relative completeness. We describe aspects of our technique that lead to useful commutativity conditions, including how predicates are selected during refinement and heuristics that impact the output shape of the condition. We have implemented our technique in a prototype open-source tool Servois. Our algorithm produces quantifier-free queries that are dispatched to a back-end SMT solver. We evaluate Servois through two case studies: (i) We synthesize commutativity conditions for a range of data structures including Set, HashTable, Accumulator, Counter, and Stack. (ii) We consider an Ethereum smart contract called BlockKing, and show that Servois can detect serious concurrency-related vulnerabilities and guide developers to construct robust and efficient implementations.

==> liftcounter.tex <==
%auto-ignore
\subsection{Lifting a Counter}
\label{apx:liftcounter}

\ktodo{here.}


==> listings/preamble.tex <==
%auto-ignore
\usepackage[utf8]{inputenc}
\usepackage[HTML]{xcolor}
\pagecolor[HTML]{FFFFFF}
\color[HTML]{000000}


==> listings/queue.tex <==
%auto-ignore
{\ttfamily\noindent
\textcolor[HTML]{0000C0}{\char35{}\enskip{}\enskip{}Queue\enskip{}definition}\\
\\
\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{queue}\\
\textcolor[HTML]{008080}{preamble}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}|}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{000000}{(declare-sort}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{0)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{000000}{(define-fun}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{valid\char95{}state}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{Int)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(front}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(nextToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(twoToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(threeToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(threeToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(twoToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(nextToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(rear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{Bool}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(or}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{0)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(and}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{1)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear))}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(and}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{2)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToRear)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear))}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(and}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{3)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToRear)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToRear)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear))}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(and}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{4)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToRear)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToRear)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToRear)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear))}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(>}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{4))}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\\
\textcolor[HTML]{008080}{state}\textcolor[HTML]{C000C0}{:}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{Int}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToFront}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToFront}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToFront}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToRear}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToRear}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToRear}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\\
\\
\textcolor[HTML]{008080}{states\char95{}equal}\textcolor[HTML]{C000C0}{:}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{008080}{definition}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}|}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(and}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size\char95{}1}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size\char95{}2)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=>}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(>=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size\char95{}1}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{1)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(and}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front\char95{}1}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front\char95{}2)}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear\char95{}1}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear\char95{}2)))}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=>}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(>=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size\char95{}1}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{2)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(and}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToFront\char95{}1}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToFront\char95{}2)}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToRear\char95{}1}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToRear\char95{}2))))}\\
\\
\textcolor[HTML]{008080}{methods}\textcolor[HTML]{C000C0}{:}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{push}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{args}\textcolor[HTML]{C000C0}{:}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{v}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{return}\textcolor[HTML]{C000C0}{:}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{result}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{Bool}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{requires}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}|}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(valid\char95{}state}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{ensures}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}|}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(and}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size\char95{}new}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(+}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{1))}\\
\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{front}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToFront\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{nextToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToFront\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{twoToFront}\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToFront\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{threeToFront)}\\
\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{v}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToRear\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{rear}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToRear\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{nextToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToRear\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{twoToRear}\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{result}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C00000}{true}\textcolor[HTML]{000000}{))}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{terms}\textcolor[HTML]{C000C0}{:}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{Int}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C000C0}{\char91{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{C00000}{1}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{(+}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{1)}\textcolor[HTML]{C000C0}{\char93{}}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{E}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C000C0}{\char91{}}\textcolor[HTML]{000000}{front}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{nextToFront}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{twoToFront}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{threeToFront}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{rear}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{nextToRear}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{twoToRear}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{threeToRear}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{\char36{}1}\textcolor[HTML]{C000C0}{\char93{}}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{pop}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{args}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C000C0}{\char91{}\char93{}}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{return}\textcolor[HTML]{C000C0}{:}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{result}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{E}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{requires}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}|}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(and}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(valid\char95{}state}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToFront}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(>}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{0))}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{ensures}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}|}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(and}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size\char95{}new}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{(-}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{1))}\\
\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{rear\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{rear}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToRear\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{nextToRear}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToRear\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{twoToRear}\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToRear\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{threeToRear)}\\
\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{front}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{result}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{nextToFront}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{front\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{twoToFront}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{nextToFront\char95{}new}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{(=}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{threeToFront}\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{000000}{twoToFront\char95{}new}\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{000000}{)}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{)}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{terms}\textcolor[HTML]{C000C0}{:}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{Int}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C000C0}{\char91{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{C00000}{1}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{(-}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{size}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{000000}{1)}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{C00000}{0}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{C00000}{2}\textcolor[HTML]{C000C0}{\char93{}}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{E}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C000C0}{\char91{}}\textcolor[HTML]{000000}{front}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{nextToFront}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{twoToFront}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{threeToFront}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{rear}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{nextToRear}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{twoToRear}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{threeToRear}\textcolor[HTML]{C000C0}{\char93{}}\\
\\
\textcolor[HTML]{008080}{predicates}\textcolor[HTML]{C000C0}{:}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C00000}{"}\textcolor[HTML]{C00000}{=}\textcolor[HTML]{C00000}{"}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C000C0}{\char91{}}\textcolor[HTML]{000000}{Int}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{Int}\textcolor[HTML]{C000C0}{\char93{}}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C00000}{"}\textcolor[HTML]{C00000}{=}\textcolor[HTML]{C00000}{"}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C000C0}{\char91{}}\textcolor[HTML]{000000}{E}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{E}\textcolor[HTML]{C000C0}{\char93{}}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}}\textcolor[HTML]{AF5F00}{-\enskip{}}\textcolor[HTML]{008080}{name}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C00000}{"}\textcolor[HTML]{C00000}{>=}\textcolor[HTML]{C00000}{"}\\
\textcolor[HTML]{000000}{\enskip{}\enskip{}\enskip{}\enskip{}}\textcolor[HTML]{008080}{type}\textcolor[HTML]{C000C0}{:}\textcolor[HTML]{000000}{\enskip{}}\textcolor[HTML]{C000C0}{\char91{}}\textcolor[HTML]{000000}{Int}\textcolor[HTML]{000000}{,\enskip{}}\textcolor[HTML]{000000}{Int}\textcolor[HTML]{C000C0}{\char93{}}\\

}

